Taming Throughput-Latency Tradeoff in LLM Inference with Sarathi-Serve

Each LLM serving request goes through two phases. The first is prefill which processes the entire input prompt and produces the first output token and the second is decode which generates the rest of output tokens, one-at-a-time. Prefill iterations have high latency but saturate GPU compute due to parallel processing of the input prompt. In contrast, decode iterations have low latency but also low compute utilization because a decode iteration processes only a single token per request. This makes batching highly effective for decodes and consequently for overall throughput. However, batching multiple requests leads to an interleaving of prefill and decode iterations which makes it challenging to achieve both high throughput and low latency. We introduce an efficient LLM inference scheduler, Sarathi-Serve, to address this throughput-latency tradeoff. Sarathi-Serve introduces chunked-prefills which splits a prefill request into near equal sized chunks and creates stall-free schedules that adds new requests in a batch without pausing ongoing decodes. Stall-free scheduling unlocks the opportunity to improve throughput with large batch sizes while minimizing the effect of batching on latency. Furthermore, uniform batches in Sarathi-Serve ameliorate the imbalance between iterations resulting in minimal pipeline bubbles. Our techniques yield significant improvements in inference performance across models and hardware under tail latency constraints. For Mistral-7B on single A100 GPUs, we achieve 2.6x higher serving capacity and up to 3.7x higher serving capacity for the Yi-34B model on two A100 GPUs as compared to vLLM. When used with pipeline parallelism on Falcon-180B, Sarathi-Serve provides up to 5.6x gain in the end-to-end serving capacity. The source code for Sarathi-Serve is available at https://github.com/microsoft/sarathi-serve.

==> 2-background-old.tex <==
\section{Background}
\label{sec:background}

LLMs stack multiple transformer blocks~\cite{attentionpaper} as their key architectural module. This section provides a brief summary of transformers and the inference procedure of LLMs.

\subsection{The Transformer Architecture}
\label{sec:background:arch}

Transformer models decompose an input query into tokens. Each of these tokens is represented by an embedding vector of dimension $h$, where $h$ is known as the embedding (or hidden) size of the model.

\noindent{\bf Self-attention module:} The self-attention module first transforms each input token via a linear transformation \attnpreproj to obtain Q (query), $K$ (key) and $V$ (value).
Next, the \attn operator computes a semantic relationship among all tokens of a sequence. This involves computing a dot-product of each $Q$ vector with $K$ vectors of all preceding tokens of the sequence, followed by a softmax operation to obtain a weight vector, which is then used to compute a weighted average of the $V$ vectors. This attention computation can be performed across multiple \textit{heads}, whose outputs are combined using another linear transformation \attnpostproj. 

\noindent{\bf Feed-forward network (FFN):}
This module consists of two linear transformations with a non-linear activation in between. The first linear layer, \ffnlnfirst, transforms an input token embedding of dimension $h$ to a higher dimension $h2$. This is followed by the activation function, typically ReLU or GELU. Finally, the second linear layer, \ffnlnsecond, transforms the token embedding back to the original dimension $h$. Note that these transformation are applied to each token of the sequence and are implemented as matrix-matrix (or vector-matrix) operations.

\noindent{\bf Other operators:} These include layer normalization, activation and residual connections. We do not discuss them in this paper as they consume only a small fraction of the overall execution time of a transformer block. \autoref{table:tensor:shapes} shows the shapes of the input, output and weight tensors of the major operators in a transformer block. 

\noindent{\bf Memory requirement:} The attention computation for each new token depends on the key ($K$), and value ($V$) tensors of all prior tokens in the sequence. To avoid recomputing $K$ and $V$ of all tokens in every iteration, most implementations cache them in GPU memory (known as KV-cache). The KV-cache size scales as $2*h*t$, where $t$ is the total number of tokens of all requests in the system, which directly depends on the context lengths of the requests and the batch size. The remaining memory is taken up by the model parameters and the intermediate activations (typically small as it can be freed after each layer). The maximum batch-size is thus determined primarily by the size of the KV-cache. As a result many recent techniques have been proposed to reduce the KV-cache size, such as multi-query attention~\cite{multiqueryattention}, grouped-query attention~\cite{groupedqueryattention}, sliding window attention~\cite{longformer} and Heavy-Hitters based attention~\cite{heavyhitters}.






\begin{table}[t]
\center
\scalebox{0.8}{
\begin{tabular}{r|2|rrr}
\multirow{2}{*}{\textbf{Operator}} & \multirow{2}{*}{\textbf{Type}} & \multicolumn{3}{c}{\textbf{Tensor shapes}} \\ \cline{3-5}
 & & Input & Weight & Output \\ \hline
\attnpreproj & linear & $[L, h]$ & $[h, h]$ & $[L, h]$ \\
\attn (prefill) & non-linear & $[l_i, h]$ & - & $[l_i, h]$ \\
\attn (decode) & non-linear & $ [1, h]$ & - & $[1, h]$ \\
\attnpostproj & linear & $[L, h]$ & $[h, h]$ & $[L, h]$ \\
\ffnlnfirst & linear & $[L, h]$ & $[h2, h]$ & $[L, h2]$ \\
\ffnlnsecond & linear & $[L, h2]$ & $[h, h2]$ & $[L, h]$ \\ \hline
\end{tabular}}

\caption{Shapes of the input, weight, and output tensors in a transformer decoder block with iteration-level scheduling. $h$ and $h2$ denote the model's primary and secondary hidden dimensions. $l_i$ denotes the sequence length of $i^{th}$ request in the batch whereas $L$ denotes the input tokens of all requests in the batch. If batch size is $B$, then $L$=$B$ during decode since each request processes one token in a decode iteration.}
\label{table:tensor:shapes}
\end{table}

\subsection{Inference Procedure}
\label{sec:background:prefill:decode}
LLM inference consists of two distinct phases -- a \textit{prefill} phase followed by a \textit{decode} phase.

\noindent{\bf Prefill:} This phase processes the entire input prompt and produces the first output token. Since all tokens in the input prompt are processed in parallel, this phase is able to effectively saturate GPU compute and is very efficient. %


\noindent{\bf Decode:} This phase follows the \textit{prefill} phase, and generates tokens autoregressively, where the token generated in the previous step is passed through the model to generate the next token. This proceeds until a special \textit{end-of-sequence} token is generated at which point the request processing is complete. Since a \textit{decode} iteration process only a \textit{single} token for a request, it is unable to saturate GPU compute. This makes the \textit{decode} phase very inefficient unless run at a very high batch size.




Multiple requests can be batched in a single iteration to improve the execution efficiency. Since the linear operations (\attnpreproj, \attnpostproj, \ffnlnfirst, \ffnlnsecond) are applied to each token independently, all token embedding vectors can be concatenated to form a matrix which can be multiplied with the linear operator's matrix via a matrix-matrix multiplication which is much more efficient than performing individual vector-matrix multiplications for each token. Note that we can combine tokens within requests (in case of prefill) as well as across requests for these operations. While \attn can also be batched, doing so is less useful because it is a memory-bound operator~\cite{orca,flashattention}. 


\noindent{\bf Inference Scheduling:} An LLM inference scheduler has to take multiple things into account. First, the requests go through the two distinct \textit{prefill} and \textit{decode} phases. Second, the processing duration of a request cannot be determined at arrival time as the \textit{decode} phase lasts until the special \textit{end-of-sequence} token is generated. Conventional inference engines like FasterTransformer~\cite{fastertransformer} perform request-batching based scheduling \ie they pick a batch of requests and execute it until \textit{all} requests in the batch complete. While this approach reduces the operational complexity of the scheduling framework, it leads to inefficient resource utilization. Shorter requests in a batch have to be padded to match the length of the longest request which results in wasteful compute. Alternatively, iteration-level scheduling has been proposed in more recent systems like Orca~\cite{orca}, vLLM~\cite{vLLM:github}, and HuggingFace TGI ~\cite{hftgi}, where requests can dynamically enter and exit a batch after each new batch of tokens are generated. Upon entering an already running batch, a newly arrived request first computes its prefill phase before entering the decode phase. Therefore, with iteration-level scheduling, prefill and decode phases get interleaved.%














\subsection{Latency Metrics}
\label{subsec:latency_metrics}
Most LLM applications, e.g. ChatGPT~\cite{chatgpt}, claude.ai~\cite{claudeai}, Bing AI~\cite{bingai}, etc. follow the streaming model for request response, where tokens are streamed to the user as they are generated. In this context, there are two primary latency metrics of interest: TTFT (time-to-first-token) and TBT (time-between-tokens). For a given request, TTFT measures the latency of generating the first output token from the moment a request arrives in the system. This metric reflects the initial responsiveness of the model. TBT on the other hand measures the interval between the generation of consecutive tokens of a request, and affects the overall perceived fluidity of the response. In this paper, we will discuss how different scheduling strategies can impact TTFT and TBT. While existing systems~\cite{orca,vllmsosp,hftgi} optimize mainly for TTFT or may require making tradeoffs between the two metrics, \sysname can allow us to achieve low values of both TTFT and TBT simultaneously. In this paper, we focus on the median value for the TTFT since this metric is obtained only once per user request and on the 99th percentile (p99) for TBT values since every decode token results in a TBT latency value.



==> 3-motivation-old.tex <==
\section{Latency-Throughput Tradeoff in LLM Inference Scheduling}
\label{sec:motivation}

In this section, we expose some of the key inefficiencies of current LLM inference serving systems. We use the current state-of-the-art serving engine vLLM~\cite{vllmsosp} as baseline for all our experiments. Unless specified otherwise, we use Yi-34B model running on two NVIDIA A100 GPUs with 2-way tensor-parallelism (TP2) for these experiments.


\subsection{Cost Analysis of Prefill and Decode}
\label{sec:analysis:throughput}
\input{fig-tex/fig-analysis-op-breakdown}


As discussed in~\autoref{sec:background:prefill:decode}, while the \textit{prefill} phase processes all input tokens in parallel and effectively saturates GPU compute, the \textit{decode} phase processes only a single token at a time and is very inefficient. To illustrate this, we compute the per-token prefill and decode times in \autoref{fig:analysis_per_token} for different input sizes. We vary the model's input size either by varying prompt length using batch size of one (for prefill) or varying batch size (for decode). We can conclude the following from this experiment.

\noindent{\bf Takeaway-1:} \textit{A single prefill request with modest sequence length can effectively saturate GPU compute}. As can be seen in ~\autoref{fig:analysis_per_token}, the prefill throughput increases almost linearly at low sequence lengths, and saturates quickly around sequence length as low as 512 tokens. Thus, even small sequence lengths can provide enough parallelism in the prefill phase to use the GPU compute effectively. This motivates the use of \chunking in \sysname.
Note that for very long sequence lengths \eg 16K, per-token prefill time increases slightly. This is due to the cost of attention operator which grows quadratically with sequence length.

The saturation point depends the model's hidden size and deployment configuration. For example, models with higher embedding size will saturate prefill throughput at smaller sequence lengths while models deployed with large degree of tensor-parallelism will require more tokens to saturate since the amount of computation per-GPU becomes smaller.


\noindent{\bf Takeaway-2:} \textit{The decode time per token is order(s) of magnitude higher than prefill, especially at small batch sizes}. As shown in ~\autoref{fig:analysis_per_token}, at a very high decode batch size of 128, the per-token decode time is still $4.4\times$ higher than the lowest prefill time per-token. Note that the decode time per token improves almost linearly with batch size. At 16, which is in lower side of decode batch sizes, the per-token decode time is still 20X. Thus, optimizing decodes is crucial for efficient LLM inference.


\noindent{\bf Takeaway-3:} \textit{Linear operators dominate the runtime cost in transformers compared to other operators like \attn}. While attention cost grows quadratically with sequence length, linear operators still contribute more than 80\% to the total time even at high sequence lengths of 16k. Therefore, optimizing linear operators is important for improving LLM inference.


\subsection{Impact of Batching on Tail Latency}
\label{sec:latencyandstalls}



\begin{figure}[t!]
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/fig_vllm_schedule.png}
        \caption{vLLM schedule. Generation stalls due to iterations $i+1$ and $i+3$.}
        \label{fig:motivation:generationstalls:vllm}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/fig_orca_schedule.png}
        \caption{Orca schedule. Generation stalls due to iterations $i+1$ and $i+3$.}
        \label{fig:motivation:generationstalls:orca}
    \end{subfigure}
    \\
        \begin{subfigure}[b]{0.48\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/fig_sarathi_schedule.png}
        \caption{\sysname schedule. No generations stalls.}
        \label{fig:motivation:generationstalls:sarathi}
    \end{subfigure}
    \caption{A generation stall occurs when one or more prefills are scheduled in between consecutive decode iterations of a request. A, B, C, D, E and F represent different requests. Subscript d represents a decode iteration, p represents a full prefill whereas p0 and p1 represent prefill chunks of the corresponding request. vLLM (a) induces generation stalls by scheduling long prefill iterations in between decodes. Despite supporting hybrid batches, Orca (b) cannot mitigate generation stalls because the execution time of batches containing long prompts remains high. In contrast, \sysname (c) generates a schedule that guarantees no generation stalls.}
        \label{fig:motivation:generationstalls}
\end{figure}






Increasing batch size is an obvious way to improve decoding efficiency. However, there are a couple of problems with this approach. First, as discussed above, even at quite high batch sizes, decode phase is not able to saturate the GPU effectively and one may need to go to very high batch sizes. Second, and more importantly, high batch size in current serving systems can result in high tail latency for TBT (time between token generation) due to a phenomenon we call \textit{generation stalls}. We discuss generation stalls and its in impact on TBT below.


\autoref{fig:motivation:generationstalls} shows how generation stalls appear in Orca and vLLM. The example shows a timeline (left to right) of requests A-F, starting with iteration $i$. At iteration $i$, requests A, B and C are all in the decode phase. After iteration $i$ finishes, request C exits the system and a new request D arrives. At this point, Orca and vLLM schedule the next iteration $i+1$ differently. vLLM supports prefill-only or decode-only batches (see ~\autoref{fig:motivation:generationstalls:vllm}) and tries to maximize the decode batch size at all times. Therefore, in the next iteration $i+1$, it schedules the prefill of D instead of the pending decodes of requests A and B, to maximize the decode batch size of future iterations. The duration of iteration $i+1$ depends on the size of D's prompt and can be several seconds. This introduces a \textit{generation stall} for ongoing decodes of requests A and B resulting in a sudden increase in TBT. A similar stall occurs later for B and D due to iteration $i+3$ where the prefill of request F is scheduled by vLLM.

In contrast, Orca supports hybrid batches \ie it can schedule requests from the prefill and decode phases in the same iteration. Hence, it batches decodes of A and B with the prefill of D iteration $i+1$ (see ~\autoref{fig:motivation:generationstalls:orca}). However, since a prefill request with long context can take a long processing time, A and B still experience a generation stall due to iteration $i+1$. Similarly, another stall appears later at iteration $i+3$ for request D. However, compared to vLLM, B experiences one less stall in Orca as its decodes finish before the prefill of F gets scheduled (thanks to hybrid batching in iteration $i+1$).

Furthermore, note that as batch size increases, the chances of prefill request(s) getting scheduled in an iteration increases, which will in turn increases the TBT tail latency. For example, increasing the maximum batch size from four to 128 in vLLM increases the p99 latency from 40ms to 2.2 seconds for Yi-34B model (we evaluate this aspect in more detail in~\autoref{sec-eval}).




\noindent{\bf Takeaway-3:} \textit{Interleaved prefill iterations increases TBT tail latency, which gets exacerbated as batch size increases.}
The duration of generation stalls is proportional to the length of prefill sequence(s) scheduled between a request's decode iterations. This is a growing concern as the use cases for higher and higher prompt lengths continue to increase. One mechanism used by current systems to reduce the increase in TBT is by limiting the batch size opportunistically (e.g., vLLM~\cite{vLLM:github} uses a parameter \textit{max\_num\_batched\_tokens}). However, lowering batch size adversely impacts throughput, and these systems are forced to tradeoff one metric over the other depending on the desired SLOs.















==> 6-discussion.tex <==
\section{Discussion} \label{sec:discussion}
In this paper, we have comprehensively demonstrated how \sysname improves the performance of LLM inference across several models and hardware configurations. However, there are multiple challenges that require further investigation.

First, we focus only on an efficient scheduling mechanism in \sysname to improve the throughput of LLM inference. However, real-world deployments need to optimize an inference serving infrastructure simultaneously along multiple dimensions e.g., latency, queuing delays, fairness, etc. Meeting these goals with \sysname requires revisiting scheduling policies. Second, although we show what is an appropriate chunk size for a given P:D ratio, we leave it to future work to explore how to pick an optimal chunk size as it depends on several factors like the hardware, model characteristics, sequence length, and the composition of prefill-decode tokens, especially in scenarios where the P:D ratio may not be known ahead of time. Third, we make a simplistic assumption in this paper that each request in a batch has the same number of prefill and decode tokens (except the simulation experiments) whereas, in the real world, the sequence lengths can vary significantly across different LLM inference requests. Finally, we focused on sequence lengths of up to 3K, and P:D ratio in the range of 1-200. We believe that these are representative of many real-world deployments. However, there has also been an increased interest in supporting very long sequences (e.g., 10s-100s of thousands~\cite{largecontextlength}). Such large sequence lengths may pose new challenges as the cost of attention grows quadratically with the number of tokens. We are actively investigating these challenges. 






==> extras.tex <==



\if
In the previous subsection, we focused on measuring the end-to-end throughput gains of \sysname while varying the P:D ratio for the highest batch size that fits on our GPU for the given context length. In this section, we dive deeper into the peak performance gain of \sysname with different context lengths while varying the batch size from two to the maximum possible, each with two chunk sizes of 256 and 512 tokens. In all these experiments, we focus on steady-state execution scenarios where the P:D ratio is balanced. As discussed above, this allows us to measure the peak performance of \sysname. For the ease of understanding, we provide some examples of a balanced P:D state in ~\autoref{table:eval:steady-state-configs}.

~\autoref{fig:all_configs} shows the results for these experiments. In total, the six sub-figures present our results for using prefill chunk sizes of 256 (first row) and 512 (Second row), each for three context lengths of 1k (first column), 1.5k (second column) and 2k (third column) tokens each. For each configuration, we show the effect of varying prefill chunk size on different batch sizes. Further, for each run, we also show the distribution of runtime across different operations i.e., {\em preproj}, {\em attention}, {\em postproj} and {\em ffn}: runtime distribution helps us understand the source of \sysname's high throughput.

~\autoref{fig:all_configs} clearly shows the source of \sysname's high throughput. Note that \sysname batches linear operations among the prefill and decode tokens to ensure high compute and memory utilization for longer periods. Therefore, the linear operations see a significant jump of up to $1.6\times$ (see ~\autoref{fig:all_configs_1k_256}, ~\autoref{fig:all_configs_1.5k_256} and ~\autoref{fig:all_configs_2k_256}) in performance compared to the baseline. However, note that the level of improvement also depends on the P:D ratio (in other words, it depends on what fraction of time is spent in decodes). For example, a chunk size of 256 has almost $2\times$ more decodes than the chunk size of 512 for the same context length (see ~\autoref{table:eval:steady-state-configs}. This means that in configurations corresponding to  chunk size of 256, a significant fraction of time is dominated by decodes, compared to one having chunk size of 512. Similarly, all other linear operations also observe significant speed up with \sysname.

One exception to this case is the {\em attn\_post\_proj} layer whose performance drops slightly at a small batch size of two while using the prefill chunk size of 256 tokens (see ~\autoref{fig:all_configs_1k_256}, ~\autoref{fig:all_configs_1.5k_256} and ~\autoref{fig:all_configs_2k_256}). We find that there are two reasons for this: (1) {\em attn\_post\_proj} has the lowest arithmetic intensity among all the linear layers of a transformer block - as shown in ~\autoref{fig:ai}. (2) in \sysname, we allow only one prefill request at a time. These two factors limit the degree of parallelism for {\em attn\_post\_proj} due to fewer input tokens, in turn, degrading its performance slightly. 

Finally, note that \sysname pays a higher cost for the actual attention computation as discussed in ~\autoref{sec-eval-attention}. However, since attention consumes a small fraction of the overall runtime, the gains in linear operations can easily recover the lost performance of attention, delivering peak throughput gains of up to $1.33\times$. \jm{We should add the normalized attn time bar as well in Fig 10}
\fi





